Same Text, Different Numbers: The Divergence of LLM-Based Measures

Researchers increasingly use generative large language models (LLMs) to convert corporate text into empirical variables. We examine the extent to which LLM-based textual measures are invariant to model choice using thirteen measures, including sentiment, management clarity, uncertainty, answer specificity, and climate and political risk. Seven LLMs from different providers score earnings call transcripts of S&P 500 companies on these constructs. Cross-model rank correlations average only 0.52, and transcript-level differences common across providers account for only 34% of total score variation. Cross-model disagreement does not predict subsequent analyst or market disagreement, consistent with a substantial model-specific component rather than common ambiguity in the underlying disclosure. Model choice significantly affects downstream inference, with coefficient magnitudes, signs, and statistical significance varying substantially across models. Averaging across providers makes transcript rankings more stable for most constructs, but score levels remain sensitive to the models included in the ensemble. LLM-generated variables should therefore be treated as model-contingent measurements and validated across providers.

==> Assets/tables/cutoff_robustness.tex <==
\begin{table}
\centering
\small
\begin{threeparttable}
\caption{Knowledge-Cutoff Robustness: Model Cutoffs and Calls Before and After Each Cutoff}
\label{tab:cutoff_robustness}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccc}
\toprule
Provider & Knowledge cutoff & Calls pre & Calls post & Straddles?\\
\midrule
Anthropic & 2023-08 & 0 & 1,946 & No\\
OpenAI & 2023-10 & 0 & 1,946 & No\\
Mistral & 2023-10 & 0 & 1,946 & No\\
Meta (Llama) & 2023-12 & 0 & 1,946 & No\\
\textbf{Qwen} & \textbf{2024-06} & \textbf{970} & \textbf{976} & \textbf{Yes}\\
\textbf{DeepSeek} & \textbf{2024-07} & \textbf{1,242} & \textbf{704} & \textbf{Yes}\\
Google (Gemini) & 2025-01 & 1,946 & 0 & No\\
\bottomrule
\end{tabular*}
\begin{tablenotes}[flushleft]\footnotesize
\item \textit{Notes:} Sample $=$ 1,946 S\&P~500 calls scored in 2024 (2024-01-04 to 2024-12-20); cutoffs from official documentation where available, and otherwise from dated developer statements or the model catalogue of the API gateway through which the model was queried. A cutoff month is read as knowledge through its last day, so a call is post-cutoff from the first day of the following month. A model ``straddles'' if it has calls both before and after its cutoff inside the sample; Qwen (2024-06) and DeepSeek (2024-07) do, so the ``post'' windows fall in 2024 (Qwen, July--December 2024; DeepSeek, August--December 2024). The difference-in-differences estimates by construct are in Table~\ref{tab:cutoff_did_construct}.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Assets/tables/main_table_CAR01_Carhart_industry.tex <==
\begin{table}
\centering
\small
\begin{threeparttable}
\caption{Relation Between LLM scores and Market Reaction}
\label{tab:main_car01_industry}
\begin{tabular}{lccccccccccccc}
\toprule
 & \rotatebox{90}{\textit{Climate Risk}} & \rotatebox{90}{\textit{Corporate Culture}} & \rotatebox{90}{\textit{Innovation}} & \rotatebox{90}{\textit{Integrity}} & \rotatebox{90}{\textit{Management Clarity}} & \rotatebox{90}{\textit{Political Risk}} & \rotatebox{90}{\textit{Quality}} & \rotatebox{90}{\textit{Respect}} & \rotatebox{90}{\textit{Sentiment}} & \rotatebox{90}{\textit{Specificity}} & \rotatebox{90}{\textit{Specificity Ratio}} & \rotatebox{90}{\textit{Teamwork}} & \rotatebox{90}{\textit{Uncertainty}} \\[6pt]
\midrule
Mistral & 0.2 & 0.4$^{***}$ & 0.2 & 0.3$^{**}$ & 0.2 & -0.1 & 0.3$^{**}$ & 0.4$^{**}$ & 1.3$^{***}$ & 0.1 & 0.4$^{***}$ & 0.3$^{**}$ & -0.5$^{***}$ \\
 & (1.27) & (2.66) & (1.25) & (2.05) & (1.01) & (-0.84) & (2.17) & (2.46) & (7.60) & (0.95) & (2.92) & (2.13) & (-2.92) \\
Gemini & 0.0 & 0.5$^{***}$ & 0.3$^{*}$ & 0.3$^{*}$ & 0.2 & -0.0 & 0.3$^{*}$ & 0.6$^{***}$ & 1.4$^{***}$ & 0.1 & 0.2 & 0.6$^{***}$ & -0.4$^{***}$ \\
 & (0.22) & (2.68) & (1.83) & (1.76) & (0.99) & (-0.29) & (1.73) & (3.79) & (8.61) & (0.72) & (1.33) & (3.62) & (-2.85) \\
OpenAI & -0.1 & 0.5$^{***}$ & 0.3$^{*}$ & 0.4$^{**}$ & 0.1 & 0.2 & 0.4$^{**}$ & 0.4$^{***}$ & 1.1$^{***}$ & 0.1 & 0.4$^{***}$ & 0.4$^{***}$ & -0.5$^{***}$ \\
 & (-0.46) & (3.11) & (1.80) & (2.55) & (0.82) & (0.96) & (2.46) & (2.67) & (7.07) & (0.87) & (3.12) & (2.71) & (-3.80) \\
Qwen & -0.4$^{***}$ & 0.2 & 0.1 & 0.1 & -0.1 & --- & 0.1 & 0.2 & 0.9$^{***}$ & -0.1 & -0.1 & 0.2 & -0.6$^{***}$ \\
 & (-2.77) & (1.21) & (0.67) & (0.92) & (-0.92) &  & (0.50) & (1.08) & (5.60) & (-0.95) & (-0.59) & (1.63) & (-3.84) \\
Llama & -0.0 & 0.4$^{***}$ & 0.1 & 0.3$^{**}$ & 0.3$^{**}$ & -0.0 & 0.3$^{*}$ & 0.3$^{**}$ & 1.3$^{***}$ & -0.0 & 0.1 & 0.4$^{***}$ & -0.5$^{***}$ \\
 & (-0.26) & (2.75) & (0.81) & (2.01) & (2.52) & (-0.30) & (1.72) & (2.22) & (7.54) & (-0.18) & (0.36) & (2.81) & (-2.99) \\
DeepSeek & 0.1 & 0.4$^{***}$ & 0.4$^{**}$ & 0.4$^{**}$ & -0.1 & 0.0 & 0.4$^{***}$ & 0.4$^{**}$ & 1.2$^{***}$ & 0.0 & 0.1 & 0.4$^{**}$ & -0.4$^{***}$ \\
 & (0.87) & (2.68) & (2.02) & (2.31) & (-0.49) & (0.11) & (2.70) & (2.48) & (7.17) & (0.25) & (0.93) & (2.45) & (-3.00) \\
Anthropic & 0.0 & 0.4$^{**}$ & 0.1 & 0.3$^{**}$ & 0.2 & --- & 0.3$^{**}$ & 0.3$^{**}$ & 1.2$^{***}$ & 0.1 & 0.0 & 0.4$^{**}$ & -1.1$^{***}$ \\
 & (0.16) & (2.45) & (0.85) & (2.40) & (1.26) &  & (2.13) & (1.98) & (7.13) & (0.88) & (0.03) & (2.46) & (-6.97) \\
Non-LLM & 0.2 & 0.4$^{**}$ & 0.2 & 0.2 & 0.1 & 0.2$^{*}$ & 0.1 & 0.2 & 0.3 & 0.2$^{*}$ & 0.2$^{*}$ & 0.4$^{***}$ & 0.1 \\
 & (1.33) & (2.33) & (1.03) & (1.63) & (0.47) & (1.72) & (0.78) & (1.33) & (1.63) & (1.91) & (1.91) & (3.17) & (0.33) \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]\footnotesize
\item \textit{Notes:} Each cell is a separate OLS regression of Carhart 4-Factor CAR(0,1) on one provider's z-scored score for one construct, with firm controls (ln(Assets), book-to-market, Tobin's Q, SUE) and industry (one-digit SIC division, nine groups) and quarter fixed effects, on the calls with a valid score from that provider and non-missing controls. The Non-LLM measures are also standardized so the coefficients are comparable within each column. The two blank cells (marked ---) are provider--construct series excluded from the sample due to lack of variation (see Section~\ref{sec:llm_measures}). CAR is in percentage points, so each coefficient is the change in CAR associated with a one-standard-deviation increase in the provider's score. $t$-statistics in parentheses, SE clustered by firm. $^{*}\,p<0.10$; $^{**}\,p<0.05$; $^{***}\,p<0.01$.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Assets/tables/regression_dispersion_range.tex <==
\begin{table}
\centering
\small
\begin{threeparttable}
\caption{Determinants of textual measure dispersion (range-based).}
\label{tab:dispersion_range}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{4}{c}{Textual Measure Dispersion (Range)} \\
\cmidrule(lr){2-5}
 & (1) & (2) & (3) & (4) \\
\midrule
\multicolumn{5}{l}{\textit{Panel A: Firm Controls}} \\
$\ln(\text{Assets})$ & 0.0169$^{***}$ & 0.0069 & 0.0070 & 0.0112$^{*}$ \\
 & (2.63) & (1.04) & (1.06) & (1.76) \\
Book-to-Market & 0.0108 & -0.0090 & -0.0092 & -0.0191 \\
 & (0.38) & (-0.29) & (-0.29) & (-0.70) \\
Tobin's $Q$ & 0.0065$^{**}$ & 0.0094$^{***}$ & 0.0092$^{***}$ & 0.0123$^{***}$ \\
 & (2.38) & (3.52) & (3.46) & (4.65) \\
SUE & -0.0032 & -0.0011 & -0.0011 & 0.0008 \\
 & (-1.57) & (-0.54) & (-0.53) & (0.39) \\
\multicolumn{5}{l}{\textit{Panel B: Textual Controls}} \\
Fog Index &  &  & -0.0074 & 0.0038 \\
 &  &  & (-0.78) & (0.39) \\
$\ln(\text{Word Count})$ &  &  &  & -0.0828$^{***}$ \\
 &  &  &  & (-3.17) \\
Financial Jargon &  &  &  & -1.0921 \\
 &  &  &  & (-1.37) \\
Numbers &  &  &  & 1.8590 \\
 &  &  &  & (1.42) \\
Forward-Looking Language &  &  &  & 1.9736$^{***}$ \\
 &  &  &  & (2.94) \\
Justification Similarity &  &  &  & -1.7357$^{***}$ \\
 &  &  &  & (-14.77) \\
\midrule
FE & -- & Industry & Industry & Industry \\
Quarter FE & No & Yes & Yes & Yes \\
Construct FE & Yes & Yes & Yes & Yes \\
Observations & 24,622 & 24,622 & 24,622 & 24,622 \\
Adj.\ $R^2$ & 0.196 & 0.199 & 0.199 & 0.217 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]\footnotesize
\item \textit{Notes:} Each column is an OLS regression at the call--construct level (1,894 calls with non-missing controls $\times$ 13 constructs). The dependent variable is LLM dispersion: the range (maximum minus minimum) across the providers of the provider-standardized LLM score for that call and construct (over the providers with a valid score for that call and construct). Controls: ln(Assets), book-to-market, Tobin's Q, SUE (winsorized at 1/99\%), the Fog index, ln(Word Count), and the financial jargon, numbers and forward-looking language shares of the Q\&A text, and the average pairwise cosine similarity of the seven providers' justifications. All columns include construct fixed effects; columns (2)--(4) add industry (one-digit SIC division, nine groups) and quarter fixed effects. $t$-statistics in parentheses, SE clustered by firm (497 firms). $^{*}\,p<0.10$; $^{**}\,p<0.05$; $^{***}\,p<0.01$.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Assets/tables/regression_dispersion_std.tex <==
\begin{table}
\centering
\small
\begin{threeparttable}
\caption{Determinants of textual measure dispersion (standard deviation).}
\label{tab:dispersion_std}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{4}{c}{Textual Measure Dispersion (Std.\ Dev.)} \\
\cmidrule(lr){2-5}
 & (1) & (2) & (3) & (4) \\
\midrule
\multicolumn{5}{l}{\textit{Panel A: Firm Controls}} \\
$\ln(\text{Assets})$ & 0.0067$^{***}$ & 0.0029 & 0.0030 & 0.0046$^{**}$ \\
 & (2.85) & (1.22) & (1.24) & (2.01) \\
Book-to-Market & 0.0028 & -0.0050 & -0.0051 & -0.0092 \\
 & (0.27) & (-0.43) & (-0.44) & (-0.94) \\
Tobin's $Q$ & 0.0019$^{*}$ & 0.0031$^{***}$ & 0.0030$^{***}$ & 0.0043$^{***}$ \\
 & (1.91) & (3.16) & (3.09) & (4.51) \\
SUE & -0.0012 & -0.0004 & -0.0004 & 0.0004 \\
 & (-1.60) & (-0.52) & (-0.51) & (0.56) \\
\multicolumn{5}{l}{\textit{Panel B: Textual Controls}} \\
Fog Index &  &  & -0.0032 & 0.0010 \\
 &  &  & (-0.97) & (0.28) \\
$\ln(\text{Word Count})$ &  &  &  & -0.0303$^{***}$ \\
 &  &  &  & (-3.34) \\
Financial Jargon &  &  &  & -0.3115 \\
 &  &  &  & (-1.12) \\
Numbers &  &  &  & 0.6018 \\
 &  &  &  & (1.31) \\
Forward-Looking Language &  &  &  & 0.7468$^{***}$ \\
 &  &  &  & (3.14) \\
Justification Similarity &  &  &  & -0.7405$^{***}$ \\
 &  &  &  & (-16.92) \\
\midrule
FE & -- & Industry & Industry & Industry \\
Quarter FE & No & Yes & Yes & Yes \\
Construct FE & Yes & Yes & Yes & Yes \\
Observations & 24,622 & 24,622 & 24,622 & 24,622 \\
Adj.\ $R^2$ & 0.176 & 0.180 & 0.180 & 0.205 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]\footnotesize
\item \textit{Notes:} Each column is an OLS regression at the call--construct level (1,894 calls with non-missing controls $\times$ 13 constructs). The dependent variable is LLM dispersion: the standard deviation across the providers of the provider-standardized LLM score for that call and construct (over the providers with a valid score for that call and construct). Controls: ln(Assets), book-to-market, Tobin's Q, SUE (winsorized at 1/99\%), the Fog index, ln(Word Count), and the financial jargon, numbers and forward-looking language shares of the Q\&A text, and the average pairwise cosine similarity of the seven providers' justifications. All columns include construct fixed effects; columns (2)--(4) add industry (one-digit SIC division, nine groups) and quarter fixed effects. $t$-statistics in parentheses, SE clustered by firm. $^{*}\,p<0.10$; $^{**}\,p<0.05$; $^{***}\,p<0.01$.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Assets/tables/summary_stats_main.tex <==
\begin{table}
\centering
\small
\begin{threeparttable}
\caption{Summary Statistics}
\label{tab:summary_stats}
\begin{tabular}{lrrrrrrrr}
\toprule
 & N & Mean & Std & Min & P25 & Median & P75 & Max \\
\midrule
\multicolumn{9}{l}{\textit{LLM-related variables (call $\times$ construct level)}} \\[2pt]
\quad LLM Dispersion (Z) & 25,298 & 0.618 & 0.315 & 0.067 & 0.415 & 0.583 & 0.784 & 2.787 \\
\quad Justif. Cosine Sim & 25,298 & 0.618 & 0.102 & 0.204 & 0.564 & 0.624 & 0.682 & 0.931 \\
\quad Justif. Jaccard Sim & 25,298 & 0.183 & 0.061 & 0.010 & 0.150 & 0.169 & 0.193 & 0.584 \\
\addlinespace
\multicolumn{9}{l}{\textit{Firm-level variables (call level)}} \\[2pt]
\quad ln(Assets) & 1,945 & 10.348 & 1.281 & 7.288 & 9.498 & 10.246 & 11.102 & 15.253 \\
\quad Book-to-Market & 1,942 & 0.328 & 0.308 & -0.638 & 0.114 & 0.257 & 0.483 & 2.380 \\
\quad Tobin's Q & 1,942 & 2.892 & 2.713 & 0.760 & 1.346 & 1.961 & 3.386 & 34.202 \\
\quad SUE & 1,898 & 2.107 & 3.177 & -5.769 & 0.279 & 1.634 & 3.300 & 14.696 \\
\quad CAR(0,1) & 1,935 & 0.020 & 6.542 & -20.733 & -3.921 & -0.106 & 4.066 & 17.321 \\
\quad Analyst Disp. (Q1) & 1,935 & 0.070 & 0.103 & 0.003 & 0.019 & 0.037 & 0.076 & 0.693 \\
\quad Analyst Count (Q1) & 1,937 & 15.126 & 6.579 & 3.000 & 11.000 & 15.000 & 19.000 & 36.000 \\
\quad Pre-Call Analyst Disp. & 1,933 & 0.071 & 0.111 & 0.003 & 0.019 & 0.037 & 0.074 & 0.799 \\
\quad Pre-Call Analyst Count & 1,934 & 15.989 & 6.421 & 4.000 & 11.000 & 16.000 & 20.000 & 38.000 \\
\addlinespace
\multicolumn{9}{l}{\textit{Textual variables (call level)}} \\[2pt]
\quad Fog Index & 1,946 & 7.381 & 0.836 & 5.112 & 6.809 & 7.301 & 7.868 & 11.633 \\
\quad ln(Word Count) & 1,946 & 8.243 & 0.352 & 4.682 & 8.067 & 8.278 & 8.461 & 9.091 \\
\quad Financial Jargon & 1,946 & 0.063 & 0.011 & 0.032 & 0.056 & 0.063 & 0.070 & 0.110 \\
\quad Numbers & 1,946 & 0.012 & 0.005 & 0.000 & 0.008 & 0.011 & 0.015 & 0.036 \\
\quad Forward-Looking & 1,946 & 0.057 & 0.012 & 0.023 & 0.049 & 0.056 & 0.064 & 0.187 \\
\quad Specificity & 1,946 & 0.013 & 0.004 & 0.004 & 0.011 & 0.013 & 0.016 & 0.040 \\
\addlinespace
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]\footnotesize
\item \textit{Notes:} The sample consists of the question-and-answer sections of 1,946 earnings calls held by S\&P~500 firms in 2024, each scored on 13 constructs by 7 LLM providers. LLM-related variables are measured at the call$\times$construct level; firm-level and textual variables are measured once per call, and their statistics are computed on the call-level panel. Variable definitions appear in Table~\ref{tab:varlist}. Per-construct summary statistics of the individual providers' z-scored LLM scores are reported in the Online Appendix (Table~\ref{tab:summary_stats_full}).
\end{tablenotes}
\end{threeparttable}
\end{table}

